Recover as It is Designed to Be: Recovering from Compatibility Mobile App Crashes by Reusing User Flows

Android OS is severely fragmented by API updates and device vendors' OS customization, creating a market condition where vastly different OS versions coexist. This gives rise to compatibility crash problems where Android apps crash on certain Android versions but not on others. Although well-known, this problem is extremely challenging for app developers to overcome due to the sheer number of Android versions in the market that must be tested. We present RecoFlow, a framework for enabling app developers to automatically recover an app from a crash by programming user flows with our API and visual tools. RecoFlow tracks app feature usage with the user flows on user devices and recovers an app from a crash by replaying UI actions of the app feature disrupted by the crash. To prevent recurring compatibility crashes, RecoFlow executes a previously crashed app in compatibility mode that is enabled by our novel Android OS virtualization technique. Our evaluation with professional Android developers shows that our API and tools are easy to use and effective in recovering from compatibility crashes.

==> src/01_intro_v1.tex <==

\section{Introduction}

% Developers have to resolve users' crash experience immediately but buts that are difficult to reproduce and fix is pain. 
% Bugs that are difficult to 

% App crash critically damages app retention. Almost 50 \% of app users delete an app when it crashes. Therefore, app developers spend a significant amount of ($>$ 50\% of development budget) dev. resources for removing app bugs before every app release, and they use automatic crash report services (e.g., Crashlytics) to fix crashes found after release quickly. However, not every bug is detected before a release, and not every bug is easily debuggable. Compatibility crash bugs are one of those kinds for Android apps. Android is a mobile OS that supports the widest range of mobile devices from low-end smartphones to high-end foldable phones. Since it's challenging for a single OS to fit all device models, Android allows device manufacturers to customize Android. For example, device vendors can lower animation quality for a low-end smartphone model and they can make Android adjust UI when their foldable phone is folded. The problem is, during customization, they add, modify, remove, and accidentally break Android OS API. Therefore, when an app is deployed to an OS with an incompatible API, the app could be crashed. 


Android OS and apps have been struggling with app crashes.
%since the first Android app was downloaded on a user device.
%\dk{The same with other software,} an Android app sometimes crashes when it goes into an undefined state due to a bug or a certain execution environment (\eg{} an outdated OS version). 
% When an app walks into a certain state that has not been tested during the development stage, the app may crash. 
% Not every bug crashes an app, but once it happens, an
% When an app crashes on a user device, an ongoing app task that user was doing on the app 
An app crash frustrates users by disrupting their ongoing tasks
Particularly, an app crash damages the app's retention% App crashes have been a serious threat to Android as they significantly damage Android apps' user experience (UX) and retention
---50\% of users that experienced an app crash delete the app~\cite{ux_damage}.
To reduce the (\ie{} crash rate), Android app ecosystem stakeholders %(i.e., app developers, Android Open Source Project (AOSP) that maintains Android OS, and third-party app libraries) 
have put in significant efforts; App developers typically target a very low crash rate ($<$ 0.5\%)~\cite{CrashFre60:online, Acceptab58:online} and spend 25-35\% of the development costs for app testing~\cite{AppDevel89:online}.
% Since \dk{app crashes also deteriorate users' overall Android experience}, 
% Android Open Source Project (AOSP) and third-party crash reporting libraries assist app developers to detect potential app crashes before app release and reproduce app crashes on user devices, respectively. AOSP maintains Android OS and develops app development tools (\eg{} Android SDK) for app developers. Therefore, they assist app developers to detect potential app crashes.
% AOSP provides a built-in app testing framework~\cite{ } and static app analysis tools~\cite{ }.
AOSP~(Android Open Source Project), which maintains Android OS, embeds an app testing framework~\cite{Espresso85:online} in Android SDK to assist app developers in detecting potential app crashes.
Third-party crash reporting libraries (\eg{} Crashlytics~\cite{Firebase20:online}) automatically collect app crash reports from user devices to ease app developers' crash reproduction. 

%During the last 15 years, debugging app crashes has been a crucial common goal of app developers and Android Open Source Project (AOSP) who maintains Android OS because an app crash seriously harms the app's user experience (UX) and retention---50\% of users that experienced an app crash delete the app\cite{ }. 
%A commonly targeted crash rate for an Android app is very low ($<$ 0.5\%). To meet the target crash rate, Android apps 
% \dk{To minimize the negative impact of an app crash,} app developers often target a very low crash rate (0.5\%). 

% therefore, \dk{reducing Android apps' crash rate} has been a common goal of app developers and Android Open Source Project (AOSP) who maintains Android OS.
% During the last 15 years, Android app developers have spent 25-35\% of the total development cost for app testing~\cite{ }

% However, not all potential app crashes are detected before an app release and some crahses are inter 
Despite their efforts, it is still difficult to predict, reproduce, or fix app crashes caused by incompatibility %with user device's OS,
between an app and the OS version that it runs on,
which we refer to as \emph{compatibility crashes}. Compatibility crashes are difficult to eliminate due to the open nature of Android platforms. To support 24,000 different Android device models in the market~\cite{Thereare14:online}, AOSP allows device vendors to customize Android OS for a specific device. For example, a foldable phone vendor customizes Android OS for adjusting UI layouts when the phone is folded, and a low-end device vendor customizes Android OS's animation quality for optimizing performance. When Android's yearly major version updates are released, the device vendors customize the new versions again for their devices. During AOSP's version updates and device vendors' customizations, Android OS APIs are added, modified, %deleted, and accidentally broken. % Since it is practically impossible to  %this is the largest cause of the compatibility crash. 
and deleted, often in a way that app developers do not expect and are hard to deal with.
Thus, apps occasionally crash when deployed on Android OSes that mismatch App APIs and OS APIs~\cite{ficfinder}.
% it would not be realistic for app developers to track the vendor-specific customizations performed on
% all of them and test the apps on them.
% Consequently,
% Since app developers cannot test their apps on all Android variations customized for diverse devices, compatibility crashes are difficult to predict, reproduce, and fix.
Compatibility crashes are difficult for app developers 
to predict, reproduce, and fix because it is not practically
feasible to test their apps on all Android variations  
customized for diverse devices.

\begin{figure}
    \centering
    % \includegraphics[width=\columnwidth{}]{figure/overview.pdf}
    % pdfcrop --margins "-13 0 -17 -15" overview.pdf
    \includegraphics[width=\columnwidth{}]{figure/androidx_osapps_issues.pdf}
    \vspace{-0.35in}
    \Description[Two bar graphs counting the number of compatibility issues the authors found from AndroidX library and top 50 open-source apps.]{Two bar graphs counting the number of compatibility issues the authors found from AndroidX library and top 50 open-source apps. One bar graph on the left side shows the issues by 10 different Android OS versions from Android JB to Android 12. For each version, 5 to 15 issues are found except for Android L having 22 compatibility issues and Android O having 21 compatibility issues. The other bar graph on the right side shows the issues by six different device vendors, Samsung, OnePlus, Huawei, LG, Google, and B&N. Samsung has 19 issues, OnePlus has 9 issues, and the other vendors have 5 issues each.}
    \caption{Compatibility issues found from top-50 open-source apps' issue trackers (156 issues in total) and AndroidX~\cite{AndroidX66:online}.
    %library's release notes (54 issues in total). AndroidX is a built-in library adopted by $>$99$\%$ of commodity Android apps, and it is supposed to provide API compatibility for the apps.}
    }
    \label{fig:androidx_issues}
    % \vspace{-.2in}
\end{figure}

% \begin{table}[]
%     \centering
%     \tabcaption{Fixed compatibility issues reported by  FicFinder$^*$ and CiD$^{**}$. Started date is the day either incompatible devices are released$^1$ or problematic app version is released.$^2$}
%     \vspace{-.0in}
%     \scalebox{0.75}{
%     \begin{tabular}{|l|c|c|c|c|c|c|}
%         \hline
%         \multirow{2}{*}{\textbf{App Name}} & \multicolumn{3}{c|}{\textbf{Compatibility Issue}} \\ \cline{2-4}
%         & \textbf{Affected OS} & \textbf{Started} & \textbf{Fixed} \eat{& \textbf{Duration}} \\ \hline \hline

%         % We have detected that in your app, method setSupportActionBar of android support library v7 is used in many activities. However, we have observed that invoking this method on some Samsung devices running 4.2 system will crash your app.
%         AntennaPod$^*$~\cite{AntennaPod} & Samsung's Android 4.2 & 2013/08/03$^1$ \eat{Aug 16, 2013$^2$} & 2016/04/22 \eat{& 32 months} \\ \hline
        
%         % I have found that AsyncTask.execute is used to load main dictionary and abbreviation dictionary in setMainDictionary in class Suggest. However, this API became slower on devices newer than Honeycomb. Tasks started by this API will be run sequentially in one thread instead of in real multiple threads. (Found in API guide) So that abbreviation dictionary will be loaded after loading main dictionary finished.
%         AnySoftKeyboard$^*$~\cite{AnySoftKeyboard} & Android 4.0 or above & 2013/05/20$^2$ & 2016/05/07 \eat{& 35 months} \\ \hline

%         % I have detected that method ConnectivityManager.getBackgroundDataSetting() is used on line 108 in nu.firetech.android.pactrack.frontend.ConfigView and line 64 nu.firetech.android.pactrack.backend.ServiceStarter.
%         % However, since this method always return true after API level 14 (Noted in API Guide) and currently the minSDK version of PactrackDroid is 14 so that calling this method is actually useless.
%         % I found that PactrackDroid has been built since 2009, I think this API may be included long time ago, but now it seems to be outdated for your app.
%         PactrackDroid$^*$~\cite{PactrackDroid} & Android 4.0 or above & 2011/10/18$^1$ \eat{Sep 11, 2009$^2$} & 2016/04/28 \eat{& 54 months} \\ \hline

%         % I have found out that the method setSupportActionBar of android support library v7 is used in many activities . However, this method crashed the app on Samsung devices.
%         PocketHub$^*$~\cite{PocketHub} & Samsung's Android 4.2 & 2013/08/03$^1$ & 2016/06/04 \eat{& 34 months} \\ \hline
        
%         ShareViaHttp$^{**}$~\cite{ShareViaHttp} & Android 4.0 or below & 2015/05/31$^2$ & 2018/07/19 \eat{& 39 months} \\ \hline
%         French Calendar$^{**}$~\cite{FrenchCalendar} & Android 3.0 to 4.0 & 2016/11/27$^2$ & 2017/02/11 \eat{& 2 months} \\ \hline
%         Red Screen$^{**}$~\cite{RedScreen} & Below Android 3.0 & 2015/10/20$^2$ & 2017/02/11 \eat{& 15 months} \\ \hline

%     \end{tabular}
%     } % scalebox
%     \label{tab:compat_issue_durations}
% \end{table}

% \dkc{awkward}
Consequently, compatibility issues are found in every Android OS version and diverse vendors' devices. % and they stay on user devices for a long time 
The issues remain until app developers fix them or incompatible OS versions and devices are removed from the market. %; hence, Android app developers and AOSP need the ability to \dk{recover from and avoid compatibility crashes.}
As shown in \autoref{fig:androidx_issues}, we investigated the top 50 open-source apps that are downloaded more than a million times~\cite{F-Droid,GitHub}. % and %on two major open-source Android app hosting sites: F-Droid~\cite{F-Droid} and GitHub~\cite{GitHub}, and we
We found 99 and 57 compatibility issues due to Android version updates and vendors' OS customization, respectively. 
% Furthermore, we have found 54 compatibility issues\yj{API mismatch?} from AndroidX library that is supposed to provide OS API compatibility for Android apps (see~\cref{sec:case_study} for details).
% \yj{The following sentence seems distracting. I am OK to cut.}
% \dk{Furthermore, we found that the AndroidX library, which provides OS API compatibility for Android apps, has its own 54 compatibility issues (see~\cref{sec:case_study} for details).}
% Second, they focus on \textit{preventing} compatibility problems at development time. Although helpful, it is not
% sufficient as not all problems are detected or manifested at development time. % as evidenced by \dk{existing research work. 
FicFinder~\cite{ficfinder}, Pivot~\cite{pivot}, and CiD~\cite{cid} found 191, 10, and 7
compatibility issues from 27, 10, and 7 already-published 
% \sk{"already-published" added. Please verify.} \hjy{verified}, 
open-source Android apps, respectively. Moreover, when we examined the source code update history of the apps that fixed their compatibility issues, the issues lasted for 30 months on average. %(see \cref{tab:compat_issue_durations}).
%Until the apps' developers fixed the compatibility problems, affected end-users had to endure the issues unless they had already deleted the apps.
%This indicates that it is likely that these compatibility problems were passed on to end users.

% Compatibility crashes require a generic solution to avoid because they are created by new OS updates and device release, and they lasts long until they are fixed. 

% Compatibility crashes have been deteriorating Android user experience. (1) Comapt crash is prevalent in real apps, (2) fixing compatibility issues takes a long time, and (3) even the latest OSes still have compatibility issues.

% To keep compatibility crashes from damaging an app's user experience,
% To avoid inevitable user experience disruptions by compatibility crashes,
Since app developers cannot prevent every compatibility crash,
% Android app developers and AOSP require an app to recover from app crashes.
%Android apps require to be recovered when it crashes.
it is desirable for Android apps to recover from their crashes.
However, developing a general recovery solution for diverse apps is difficult because (1) recovering an app's state often requires custom logics specific to app internals, and (2) exisiting fault tolerance methods, such as application checkpointing~\cite{CRIU3:online}, cannot guarantee the complete elimination
of recurring crashes. Although these methods can recover an
app and restart it, the root cause of the problem still exists, leading to the possibility of further crashes.
%cannot prevent a recovered app from falling into the previous compatibility crash again.

To overcome these difficulties, we propose to adapt a well-known, user-centric app design
concept called \emph{user flow} and design a programmable abstraction around it as the basis
for a general recovery solution. User flow in UX design captures the sequence of UI actions
that a user takes to achieve a specific goal. Turning this into a programmable abstraction,
we design a system that records a user flow and replays it to perform recovery if the user
flow is interrupted by a compatibility crash. Unlike previous UI record-and-replay systems
that blindly record all UI actions, our user flow abstraction only captures the essential UI
actions required to achieve a goal to avoid unnecessary UI actions during recovery. We
provide app developers with a convenient API to express user flows in their apps and a
record-and-replay system that matches a user's UI actions with a user flow to replay it when
there is a crash.  Using user flow
is more advantageous than app state restoration because (1) it is agnostic to app internals
as it only deals with UI actions, and (2) it does not involve the restoration of app state that
may already be corrupted by compatibility issues.
%\dk{To overcome those difficulties, we propose a user-centered crash recovery solution that focuses on restoring a user's intent disrupted by a crash, instead of restoring the exact app's state.
%A mobile app user makes UI actions under an intent; therefore, if we can capture user intents on user devices in real-time, we can recover a disrupted user intent by replaying corresponding UI actions. Our crash recovery by user intent replay is more advantageous than crash recovery by app state restoration because (1) it is agnostic to app internals as it only requires UI actions for recovery, and (2) it does not necessarily involves restoration of app state that may already be corrupted by compatibility issues. 
% \yj{Do we need the following sentence. What does it add more than the previous discussion?:
% "While there is no generic solution that captures user intents on an arbitrary app, we argue that app developers know the user intents supported by their app and the UI actions required for the intents. We thus bridge the gap by providing an easy-to-use API for app developers to express user intents in program code %that is to be 
% used for crash recovery."}
In addition, we design a new execution environment called
\emph{compatibility mode} that prevents our recovery process from encountering the same
compatibility crash, which we describe in \cref{sec:compatibility-mode}. 

To demonstrate the idea, we build a crash recovery system, \proj{}, that addresses all three major challenges via UI-driven compatibility crash recovery.
The first challenge is in tracking user intents on a user device. Our API guides app developers to consider one user intent at a time and develop a user flow, which is a graph of possible UI actions to be matched for the intent. With our API and developer tool, the developers can visually program a user flow by selecting UI elements on app screens. During an app execution, \proj{} holds UI action records that match with unfinished user flows, and replays them on a crash.

The second challenge is in handling develop-time, record-time, and replay-time UI mismatches.
% A developer's crash recovery logic matching a UI action with an x-y coordinates into a user intent may fail on user devices due to screen size changes. A user's UI actions recorded before a crash may results in unpredictable outcomes when replayed after the crash due to UI changes by external causes (\eg{} network connectivity).
A user flow must robustly match UI actions against diverse user device screen sizes and possible UI changes between when UI actions are recorded before a crash and when replayed for recovery.  
To do so, \proj{} expresses an Android view of a UI action with VPath, our extended version of XPath~\cite{XPathMDN8:online} that is commonly used for web automation. A developer can customize VPaths generated by our developer tool to match a UI action with semantics; \eg{} recording a button click with text on the button instead of clicked x-y coordinates on the screen.
%We further assist the developers by providing a developer tool, which enables the visual programming of a recovery logic. %With the tool, the programmers can visually select Android views to include in a stage, and our tool generates Java code for constructing a stage with automatically suggested VPaths for the selected views.

The third challenge is in avoiding repeating the same compatibility crashes.
With \proj{}, AOSP can micro-virtualize Andorid OS on a user device and execute an app on a compatible guest Android OS, together with other apps on the host user device OS.
The key idea is (i) designating a small number of Android OS releases as \textit{compatibility OSes},
(ii) providing an execution environment that acts as a compatibility OS to resolve OS API mismatches,
and (iii) enabling an app to run on a compatibility OS execution environment when it crashes on the default OS installed on a user device.
\proj{} automatically detects an app crash, boots a compatibility OS within a few seconds~(2.5~sec on average),
and re-launches the crashed app in the compatibility OS.
% An app running in compatibility mode is transparent to the default OS as a regular app.
% Therefore, the re-launched app does not break any compatibility with running apps and the default OS's app management policy.

Our system evaluation demonstrates that \proj{} effectively recovers commodity open-source applications by replaying our user study participants' UI action traces. Our developer study participants developed app crash recovery logic for diverse app features with our API. The cost for \proj{}'s compatibility mode is small 
while it effectively hides compatibility crashes.
The \proj{}'s compatibility mode successfully avoids
compatibility crashes of one real-world app and five custom apps. 
When enabled, the \proj{}'s compatibility mode induces
only a marginal delay ($2.7\%$) to app execution with 38.7~MB 
additional memory.

We make the following contributions:
%\begin{compactitem}[\labelitemi]
\begin{enumerate}
\item \proj{} provides an API for recovering a crashed app to the state before the last crash. App developers can write easy-to-maintain recovery code with our API. %We discuss our crash recovery API further in~\cref{sec:recovery}.
\item \proj{}'s recovery API is the first API to enable on-device user intent tracking for Android apps. 
\item \proj{} is the first compatibility mode app execution framework for Android.\footnote{We will open source \proj{} with this paper's publication.}
\item \proj{} implements a novel Android OS virtualization technique
in a real system that effectively executes an app in a virtualized OS yet incurs only minimal overhead.
\end{enumerate}
%\end{compactitem}

% \sk{With sections 2 \& 3, I think it's taking too long to get to the actual meat of the work.
% It's especially because sections 2 \& 3 do not help readers understand why they need to read
% those sections. It looks to me that those sections explain important facts, which is good,
% but they don't blend together well with the overall story of the paper. I.e., they read like
% a laundry list. We probably need a different structure or a strategy.}
% \dkc{Agree with you. If we move Related Work to after Micro Benchmark, do you think the issue would be resolved?}
% \dkc{Addressed by moving related work to back}
% To do so, we provide a shell script patching existing Android OS to be capable of executing individual apps with a given OS image. When device vendors port an Android OS to new devices or update existing devices over-the-air (OTA), they can patch the devices' OS with our patch script and place a secondary Android OS image from the set in their device storage. When an app crashes on a patched OS, the OS launches the app again with the secondary OS. \dkc{must say that \proj{} is not limited to new devices, but also applicable to legacy devices that OS version updates are discontinued.}





==> src/05_micro_virt.tex <==

\section{Compatibility\,Mode\,by\,Micro\,Virtualization}
\label{sec:virtualization}

%\sk{This looks repetitive. These are included in the previous section, so we can just cut this.}
%\dk{For the compatibility mode app execution, \proj{} executes an app with the compatibility OS's app framework on the host OS. To do so, (1) the compatibility OS needs to be packaged as an image file, (2) the host OS needs to be patched to control the compatibility mode, (3) SSI translation packs need to be developed to mitigate SSI mismatches between the compatibility OS and the host OS, and (4) the two OSes and SSI translation packs work in tandem to execute the app in the compatibility mode. In this section, we discuss the technical details about those four steps except (3) that to be discussed in~\cref{sec:translation}.

We present how we enable our compatibility mode, including how we generate a compatibility
OS image, which modifications are required on a host Android OS, and how we execute an app
in our compatibility mode.

% We virtualize Android OS for an app in compatibility mode and executes the app with a compatibility OS (\ie{} guest OS) on 

%\subsection{Packaging a Compatibility OS Image}
\subsection{Generating a Compatibility OS Image}
\label{sec:disk_image}

\begin{table}[]
    \centering
    \tabcaption{Android OS modification for compatibility OS image creation.}
    % \vspace{-.0in}
    \scalebox{0.75}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        \multirow{2}{*}{\textbf{OS Release}} & \textbf{Total} & \multicolumn{3}{c|}{\textbf{Modified LoC}} \\ \cline{3-5}
        & \textbf{LoC} & \textbf{Boot script} & \textbf{Java/C/C++} & \textbf{Makefile} \\ \hline \hline
        % AOSP 4.1.1 & 27785737 & & & \\ \hline
        % cloc --diff $(git rev-parse android-4.1.1_r1) $(git rev-parse android-compat-4.1.1_r1)
        AOSP 4.1.1 & 27.7M & 207 & 37 & 39 \\ \hline
        % 48747771
        AOSP 5.0.2 & 48.7M & 250 & 55 & 22 \\ \hline
        % AOSP 8.1.0 & 67513959 & & & \\ \hline
        AOSP 8.1.0 & 67.5M & 157 & 126 & 3 \\ \hline
    \end{tabular}
    } % scalebox
    \label{tab:os_modification}
    % \vspace{-.5in}
\end{table}

The generation of a compatibility OS image is mostly automated by our \pkgtool{}. It repackages a
regular Android OS's disk images into a compatibility OS image. The tool copies everything in the
regular Android OS's images to the compatibility OS image. It then removes files unnecessary for
the compatibility OS's app execution environment, \ie{} built-in system apps, and boot scripts for unused system services. %\sk{Can we have an exact list of things here?}

% During repackaging, two types of manual efforts are required.
Although \pkgtool{} automates most of the image generation tasks, there are two tasks that are
difficult to automate and, hence must be done manually by AOSP.
%With our \pkgtool{}, AOSP has two manual tasks to do.
First, manual boot script modification is required for (1) disabling the compatibility OS's system services as the host OS's system services will be used instead, (2) disabling disk partition mounts as every file for the compatibility mode is already in the compatibility OS image, and (3) linking apps' local data directories to share the host OS's apps and their data with the compatibility OS. The required modification consists of deleting ``\texttt{mount} ...'' commands and ``\texttt{service} ...'' blocks and adding a command for bind-mounting the host OS's \texttt{/data/data} directory where all apps and their local data are stored.

%Second, manual Binder RPC library source code modification is required for injecting SSI translation hooks. For the SSI translation API, our SSI translation hook must be called when a Binder message is  
Second, manual source code modification is required for injecting SSI translation hooks. These hooks
must be injected in \textit{Binder}, which is the main inter-process communication mechanism of Android and relays every SSI call in Android.
% \sk{Check if Binder is mentioned earlier. Revise accordingly.}
%received or to be sent. We explain how it is used in \cref{sec:translation}.
In our experience of packaging three compatibility OSes, only a small number of lines had to be modified (see \cref{tab:os_modification}).



% \dkc{say that packaging is choosing copying what compose app exec env and disabling others to avoid conflicts with hsot OS. we do this for each objective. }

% \dk{Android app is incomplete by itself. It doesn't even have program entrypoint (\eg{} main function). It is basically a set of callback functions for events generated by Android OS (\eg{} app start). Android OS loads an app in its provides app execution environment.} Android OS's app execution environment has four major components: app framework, system servers, linux kernel, and file system directories. We virtualize or share \dkc{FIXME. virtualize or share??? copy to image or reuse host's} each component to meet the four objectives as described in~\cref{fig:architecture}. \dkc{And we write them in a disk image.}

% App framework is the component we must virtualize \dkc{copy?} for the first objective. App framework is a set of system libraries used by app processes. It abstracts the rest of Android OS for the app. It implements Android OS API, Java language, and core native libraries. It resolves important directory paths (\eg{} app-specific data directory) and communicates with system servers on behalf of the app. \dk{Since it implements Android API it must be virtualized} \dkc{App framework is in \texttt{system.img}. We also need \texttt{ramdisk.img} to boot guest OS and start zygote. we merge two images into one image.}

% For the second objective, we share host OS's system servers. \dkc{we modify \texttt{init.rc} and other rc files to disable all system servers except Zygote. We modify \texttt{init.rc} to bind host OS's \texttt{/dev/socket} where system servers' sockets are created at \texttt{/host} and symlinked the sockets to guest OS's \texttt{/dev/socket}.}

% For the third objective, we share file system directories. \dkc{We modify \texttt{init.rc} to bind host OS's \texttt{/data} where app-specific data directories reside and \texttt{/storage} where external SD card are mounted to \texttt{/host} and links them}

% Regarding the fourth objective, our architecture only adds minimal overhead. we do not stack software components for virtualizaiton. we replace app framework and share linux kernel and system servers. 
% % \begin{itemize}
% %     \item \textbf{App framework:} A set of system libraries essential for app execution.
% %     \item \textbf{Zygote:} A special system server that forks into an app.
% %     \item \textbf{Other system servers:} For example, window manager relays screen touch events through Linux pipe.
% %     \item \textbf{File system:} App-specific data directory, cache directory, and shared storage directory.
% % \end{itemize}

% % To achieve the three objectives at the same time, we (1) virtualize only app framework, a part of Android OS required for the first objective and (2) reuse the rest of Android OS (\eg{} system servers and Linux Kernel) for the second and the third objectives.




\subsection{Patching a Host OS}
% \dkc{we also zygote -> hygote, inject zygote-switch}

% A host Android OS on a user device launches an app in compatibility mode after a compatibility OS image is downloaded on a user device. To do so, the host OS should be able to (1) boot a compatibility OS from the image and (2) 
% When an app needs to be executed
%To execute an app
%in the compatibility mode, the host OS on a user device (1) boots a compatibility OS from a compatibility image and (2) asks the compatibility OS's Zygote to launch the app. As existing Android OSes do not have such abilities, we provide a patch for enabling them to do so. The patch needs to be executed once by the bootloader, and it requires neither modifying the host OS's source code nor installing an updated OS on a user device. 
On the host OS, we add the capability to boot a compatibility OS and launch an app in 
compatibility mode. As discussed in \cref{sec:ecosystem}, we developed a tool that applies this change as
a patch delivered to a user device as an OTA update.

%The patch performs two tasks. The first task is injecting two files to the user device's root file system.
%One is \controller{}, a shell script mounting a compatibility image and booting a compatibility OS in the mounted image.
%One is a shell script mounting a compatibility image and booting a compatibility OS in the mounted image.
% Another is \zswitch{}, our executable that hijacks a unix socket connection between activity manager and host OS's zygote. \zswitch{} usually relays activity manager's app launch requests to host OS's zygote but it redirects the requests to compatibility OS's zygote when the app needs to be in the compatibility mode.
% % so the compatibility OS's zygote can launch the app.
% Second, the patch updates an existing boot script, \texttt{init.rc}, to make \zswitch{} operate. Zygote is supposed to open a socket at a fixed path, \texttt{/dev/socket/zygote}, so activity manager can connect to it. The patch makes zygote open a socket at a different path, and it makes \zswitch{} to open a socket at the original zygote socket path. When activity manager connects to \texttt{/dev/socket/zygote}, \zswitch{} decides where to forward activity manager's app launch requests between host OS's zygote and compatibility OS's zygote. We explain more details about compatibility mode app execution in \cref{sec:execution}.
The patch performs two tasks. The first task is injecting \zswitch{} to the user device's root file system.
\zswitch{} is an executable that redirects app launch requests to the host OS's Zygote or
the compatibility OS's Zygote.
Since Zygote receives app launch requests via \texttt{/dev/socket/zygote} unix domain socket, \zswitch{}
intercepts this domain socket and distributes all app launch requests appropriately.
%an app is launched by Android's system service called Activity Manager, which
%writes an app launch request to \texttt{/dev/socket/zygote} unix domain socket. Zygote then reads each
%request from the same domain socket. Thus, \zswitch{} intercepts this domain socket from Zygote, receives
%app launch requests from it, and forwards requests to either the regular Zygote or the compatibility
%OS's Zygote, depending on the execution mode. We explain more details on compatibility mode app
%execution in \cref{sec:execution}.
\zswitch{} is also in charge of mounting a compatibility OS image and booting it (see \cref{sec:execution}).

The patch's second task is updating the existing boot script, \texttt{init.rc}.
The patch adds two commands. One is to start \zswitch{} at boot time and the other is to reconfigure the
socket paths for the regular Zygote and \zswitch{} so that \zswitch{} can intercept the original domain
socket.

% \sk{I think the total count is also important.}.
% dhkim: how we counted the lines
% 1. for C++/Java in common:
%   - excluded codes that simply mirrors host OS code. (i.e., files starting with "Host" or ending with "Mirror". 
%   - excluded dummy translators for suppressing errors we print
% 2. for C++:
%   - counted all code lines then divided it by the number of pretender, proxy, and SSI calls. 43.4 LoC/translator (= 825 LoC / (1 pretender, 3 proxies, and 15 call translators)). command: "cd ssitl/src/translators/android-4.1.1_r1-android-4.0.4_r1 && cloc cpp/input_proxy/InputProxy.* cpp/android_view_InputDeviceUpProxy.cpp cpp/IDisplayEventConnectionPretender.* cpp/InputChannelUpProxy.* cpp/IServiceManagerDownTranslator.* cpp/ISurfaceComposerDownTranslator.* cpp/ISurfaceTextureDownTranslator.* cpp/IWindowManagerDownTranslator.* cpp/IWindowSessionDownTranslator.*"
% 3. for Java:
%   - for call translators: remove generated code then count lines. manually written code: (1) interface translator structure, (2) call parameter and return value list change, (3) use of proxies. 
%   - for proxies: a proxy is mostly auto-generated except manual modifications for using other proxies.
%   - for pretenders: it's all manually written
%   - results: 9.7 Loc/translator (= 271 LoC (= 48 LoC call translators + ...) / (1 pretender, 11 proxies, and 16 call translators)
% 4. results:
%   - 23.31 (= (825 + 271) / (1 + 3 + 15 + 1 + 11 + 16))




% \dkc{we probably want to speak about AOSP and the vendors' motivations for not only translating SSI but also facilitating \proj{} ecosystem.}


\subsection{Executing a Compatibility Mode App}
\label{sec:execution}

% \dkc{how do we handle file system layout incompatibility?}
The first step in executing an app in our compatibility mode is detecting an app crash.
For this purpose, \zswitch{} monitors Android's system message dump called \texttt{logcat}
as it logs every app crash.
%When \zswitch{} detects an app crash, it initiates the compatibility mode.
%The compatibility mode is initiated when \zswitch{} detects an app crash.
%When an app crashes for any reason (\eg{} uncaught Java exception or segmentation fault from native code), the app's runtime records it to \texttt{logcat}, Android's system message dump. 
%\zswitch{} monitors logcat and it asks activity manager to launch the crashed app.
When \zswitch{} detects an app crash while monitoring \texttt{logcat}, \zswitch{} places an empty file named ``.crashed'' in the app's data directory.
\zswitch{} then uses Android's regular channel for launching an app (i.e., via a system service
called the \textit{Activity Manager}) to send a request to relaunch the crashed app. This request is ultimately
delivered to the \texttt{/dev/socket/zygote} domain socket, which \zswitch{} receives.
%If app name on the request matches with the crashed app then \zswitch{} tries to forward the request to compatibility OS's Zygote.
\zswitch{} then checks the ``.crashed'' file in the app's data directory to forward the request to compatibility OS's Zygote if the file exists.
%However, forwarding the request may fail if the compatibility OS's Zygote is not running. In that case, \zswitch{} boots the compatibility OS and does busy-waiting until the compatibility OS's Zygote opens the unix socket for receiving the request.
When the app is crashed for the first time and there is no compatibility OS running, \zswitch{} first boots the
compatibility OS.
%forwarding the request may fail if the compatibility OS's Zygote is not running. In that case, \zswitch{} boots the compatibility OS and does busy-waiting until the compatibility OS's Zygote opens the unix socket for receiving the request.
% \dkc{TODO: ask SJ to explain how to detect crash. We need to know how to clear crash indicator file for unmodified apps.}

%To boot the compatibility OS, \zswitch{} executes \controller{}. \controller{} mounts a compatibility OS image using \texttt{chroot} into a mount point, and starts the compatibility OS's init script. The init script sets up Linux environment variables, bind-mounts required host OS directories (\eg{} app-local data directories), and starts compatibility OS's Zygote. 
To boot the compatibility OS, \zswitch{} mounts a compatibility OS image using \texttt{chroot} into a mount point and starts the compatibility OS's init script. The init script sets up Linux environment variables, mounts required host OS directories (\eg{} app-local data directories), and starts compatibility OS's Zygote. 
% The Zygote forks and specializes into the app when it receives the request.
After compatibility OS's Zygote is started, it finally receives the app launch request, and it forks and specializes into the app.

%During an app execution, compatibility OS's app framework in the app works together with host OS's system services via SSI. Whenever the app framework receives or sends a Binder message for an SSI call, SSI translation hook is called for translating the call with SSI translation packs. We explain SSI translation details in \cref{sec:translation}.
During an app execution, the compatibility OS uses the host OS's system services. Since Android
uses Binder to communicate between an app and the system
services, we intercept Binder messages to redirect the communication between the host OS's
system services and the app running on the compatibility OS (see
\cref{sec:translation}).
%is that whenever the app framework receives or sends a Binder message for an SSI call, SSI translation hook is called for translating the call with SSI translation packs. We explain SSI translation details in \cref{sec:translation}.
% If the app is developed with \libsc{} and it enables the crash recovery
%
In addition, an app developer can optionally use our crash recovery library (\libsc{}) to
customize how recovery should be handled (see \cref{sec:recovery}).
%If the app uses \libsc{} and crash recovery is enabled for the app
%then \libsc{} restores the app's context by replaying the last UI actions before a crash. We discuss our crash recovery details in \cref{sec:recovery}.

% \noindent\textbf{Creating compatibility OS image:} 

% \noindent\textbf{Virtualizing file system with \texttt{chroot}:} 

% \noindent\textbf{Sharing Kernel and system services:} 

% Others include environment variables, 

% % \subsection{\libsc{}}

% \subsection{Compatibility OS Image Compression}



==> src/06_translation.tex <==
\section{System Service Interface Translation}
\label{sec:translation}

In \proj{}, a compatibility OS uses the system services of the host OS, which means that
it uses the system services from a different OS version. This naturally creates a possibility of
interface mismatch, \ie{} the interface of the host OS's system services might be different
from what the compatibility OS expects.

To illustrate this problem, consider a compatibility OS based on AOSP's \texttt{android-9.0.0\_r1}
(Pie) and a host OS based on \texttt{android-8.1.0\_r74} (Oreo). Android Pie allows an Android device
to have multiple Ethernet ports while Android Oreo allows at most one Ethernet port. Therefore, the
Ethernet Manager system service in Pie requires an interface name parameter for an Ethernet port (\eg{}
\texttt{boolean isAvailable(String interface)}) while Oreo\eat{\texttt{8.1}} does not (\eg{}
\texttt{boolean isAvailable()}).

To address this problem, \proj{} translates system service interface (SSI) calls at run time.
Since an SSI mismatch occurs due to AOSP's OS updates and vendors' OS customizations, \proj{} asks AOSP
and vendors to write their own SSI translation for their SSI changes. Since this process of writing
interface translation could be tedious, \proj{} provides an \codegen{} that automates many aspects of
the process. %, which we detail in this section.

\subsection{Translation Code Generation}
\label{sec:translation-code-generation}

To gain insights on SSI translation before developing a translation code generation tool,
we manually translated 47 SSI calls between a compatibility OS based on Android Jelly Bean
and a host OS based on Android Ice Cream Sandwich. This experience revealed that there are five mismatch
\textit{patterns} that generally capture how a mismatch could occur. %Although we do not claim that this is a definitive study, we observed that 
All 47 SSI calls that we manually translated fall within
one of the five patterns or a combination of them.
% \sk{What do we do for cases outside of these patterns?}
%\dk{We note that directly modifying RPC messages for translating an SSI call is always possible regardless of the patterns.}
We found that translations could be fully automated for some patterns, but 
certain patterns are difficult to be fully automated. Thus, our translation code generation tool
aims to provide as much automation support as possible. Though we do not currently provide
automation support outside of the five patterns, we note that AOSP or vendors can always
manually translate an SSI call regardless of the patterns. The following are the five patterns
and how our automation support handles each pattern.

% \begin{figure}[!t]
%     \centering
%     % \begin{subfigure}[b]{\columnwidth{}}
%     %     \centering
%         % \scalebox{0.90}{
%         \lstset{basicstyle={\scriptsize\ttfamily},
%                 keywordstyle=\bfseries\color{blue},
%                 stringstyle=\bfseries\color{olive},
%                 commentstyle=\bfseries\color{gray},
%                 morecomment=[s][\color{gray}]{@}{\ },
%                 numbers=left,
%                 aboveskip=0pt,
%                 belowskip=0pt}
% %         \lstinputlisting[language=Java,lastline=1]{code/call_translator.txt}
% %         \lstinputlisting[language=Java,firstnumber=2,firstline=2,lastline=2,backgroundcolor=\color{orange!10}]{code/call_translator.txt}
% %         \lstinputlisting[language=Java,firstnumber=3,firstline=3,lastline=3]{code/call_translator.txt}
% %         \lstinputlisting[language=Java,firstnumber=4,firstline=4,lastline=9,backgroundcolor=\color{orange!10}]{code/call_translator.txt}
% %         \lstinputlisting[language=Java,firstnumber=10,firstline=10,lastline=26]{code/call_translator.txt}
% %         \lstinputlisting[language=Java,firstnumber=27,firstline=27,lastline=29,backgroundcolor=\color{orange!10}]{code/call_translator.txt}
% %         \lstinputlisting[language=Java,firstnumber=30,firstline=30]{code/call_translator.txt}
% %         % } %scalebox

%         % \lstinputlisting[language=Java,lastline=2]{code/call_translator_v2.txt}
%         % \lstinputlisting[language=Java,firstnumber=3,firstline=3,lastline=3,backgroundcolor=\color{orange!10}]{code/call_translator_v2.txt}
%         % \lstinputlisting[language=Java,firstnumber=4,firstline=4,lastline=4]{code/call_translator_v2.txt}
%         % \lstinputlisting[language=Java,firstnumber=5,firstline=5,lastline=11,backgroundcolor=\color{orange!10}]{code/call_translator_v2.txt}
%         % \lstinputlisting[language=Java,firstnumber=12,firstline=12,lastline=13]{code/call_translator_v2.txt}
%         % \lstinputlisting[language=Java,firstnumber=14,firstline=14,lastline=16,backgroundcolor=\color{orange!10}]{code/call_translator_v2.txt}
%         % \lstinputlisting[language=Java,firstnumber=17,firstline=17]{code/call_translator_v2.txt}
        
%         \lstinputlisting[language=Java,lastline=2]{code/call_translator_v3.txt}
%         \lstinputlisting[language=Java,firstnumber=3,firstline=3,lastline=3,backgroundcolor=\color{orange!10}]{code/call_translator_v3.txt}
%         \lstinputlisting[language=Java,firstnumber=4,firstline=4,lastline=4]{code/call_translator_v3.txt}
%         \lstinputlisting[language=Java,firstnumber=5,firstline=5,lastline=11,backgroundcolor=\color{orange!10}]{code/call_translator_v3.txt}
%         \lstinputlisting[language=Java,firstnumber=12,firstline=12,lastline=13]{code/call_translator_v3.txt}
%         \lstinputlisting[language=Java,firstnumber=14,firstline=14,lastline=16,backgroundcolor=\color{orange!10}]{code/call_translator_v3.txt}
%         \lstinputlisting[language=Java,firstnumber=17,firstline=17]{code/call_translator_v3.txt}

%         % } %scalebox
%         % \caption{ for opening default DB file using KeePassDroid.}
%         \label{fig:api_snippet}
%     % \end{subfigure}
%     % \hfill
% %     \caption{A SSI call translator code for translating Android 9.0 OS's \texttt{isAvailable(String ifname)} to Android 8.1 OS's \texttt{isAvailable()}. Only the highlighted lines are manually written, otherwise automatically generated, and more generated code is omitted.}

%     \caption{A Java SSI call translator code for translating Android 9.0's \texttt{isAvailable(String ifname)} to Android 8.1's \texttt{isAvailable()}. Only the highlighted lines are manually written, otherwise automatically generated, and more generated code is omitted.
%     \sk{I think this example is not highlighting what exactly a developer needs to do well enough.
%     Is there a better way?}
%     }
%     \label{fig:api_example}
    
% \end{figure}

%\begin{enumerate}[leftmargin=2\parindent]
%    \item 
\noindent \textbf{1. Inconsistent call ID:}
    % \dkc{we do this automatically}
    An SSI call is essentially an RPC call and there is an ID for a target remote (system service)
    method. This call ID of each SSI call is usually hard-coded in the source code, and the same SSI
    call in two different Android OS versions might have different call IDs due to source code updates.
    Thus, one frequent pattern of mismatch is using a wrong call ID. However, we found that
    resolving this is easy and can be fully automated for the methods that preserve
    their method name across versions, as we only need to translate call numbers. Thus, our
    \codegen{} supports fully automated translation of call numbers.

 %   \item 
\noindent \textbf{2. Inconsistent Parcel definition:} 
    % \dkc{we generate converter}
    An SSI call's arguments and return values are transported via object serialization, and Android uses
    an object format called Parcel. However, Parcel can be customized by
    implementing \texttt{writeToParcel()} and \texttt{createFromParcel()}, which might change across
    versions. Thus, it is another mismatch pattern that SSI translation must handle. We found that this translation could also be fully automated as we can read a Parcel
    with one SSI's \texttt{createFromParcel()} method and write it with another SSI's
    \texttt{writeToParcel()} method. Thus, our \codegen{} supports fully automated translation of
    Parcels.
    
%    \item 
\noindent \textbf{3. Inconsistent call signature:}
    % \dkc{we generate call translator}
    An SSI call's parameters and return values might change across versions, which is another mismatch
    pattern. Our previous example of the \texttt{isAvailable()} method belongs to this pattern
    as it requires dropping of the \texttt{String interface} parameter. In general, this requires a
    semantic understanding of interface differences and thus is difficult to fully automate. Our \codegen{} provides automation support where it identifies mismatches in the method signature
    (\eg{} parameters or return value) and generates a code template that a developer could use to fill
    out parameter or return value translation.
    \dk{The code templates fills missing parameters with default values (\eg{} 0 for int type parameters), and a developer can change the values if necessary.}
    % Figure~\ref{fig:api_example} shows an example of
    % translating a \texttt{isAvailable} SSI call.
    % \sk{Some discussion/numbers about how effective this is.}
    In our translation experience, the code generation tool generated 1,007 lines out of 1,055 lines of Java code translating 16 SSI calls' call signature.
    
%    \item 
\noindent \textbf{4. Non-existent system service object:} 
    % \dkc{should create pretender}
    % \sk{A test double or a mock object is a standard term used in testing for these kinds of things.
    % Perhaps something along those lines might be appropriate here as well.}
    When an app uses a system service, it obtains a handle for the system service in the form
    of a Java object. The app then makes SSI calls using the object. However, these Java objects
    might not be available as the corresponding system services could be added or removed across versions.
    % \sk{What exactly are the cases here? System service name change? Number change? Removal? Or all
    % of these and more?}
    Thus, our \codegen{} creates a code template to handle such cases. By default, our template 
    returns an error notifying the caller that the system service is unavailable. However, AOSP and
    vendors can customize our template to return a mock system service
    % \sk{or a mock system service}
    that handles the calls more gracefully.
    % For example, \sk{I think we need to give some sense of what
    % they can do.}
    For example, Jelly Bean OS introduced the \textit{Input Manager}, a new system service taking over the
    input event management task (\eg{} the keyboard input) from the \textit{Display Manager} system service. For translating a \texttt{getInputDevice()} SSI call from a Jelly Bean compatibility OS, we created a mock Input Manager object delegating the call to the Display Manager's \texttt{getInputDevice()} for an Ice Cream Sandwich host OS.
    % \sk{Give some experience description here, how many lines, was it difficult, etc.}
    It took only 8 lines of Java code for delegating the call and 105 lines for the entire mock Input Manager.
    
%    \item 
\noindent \textbf{5. Non-existent SSI call:} 
    % \dkc{alternative reply}
    %When destination SSI does not have a SSI call invoked from source SSI, a call translator should make a reply message on behalf of destination SSI. To do so, the call translator should drop transaction message by returning \texttt{null} from \texttt{translateTransaction()} method, and compose the reply message in \texttt{translateReply()} method.
    % \sk{I wasn't too sure about this.}
    Sometimes SSI methods are removed across versions, which we handle in a similar fashion as the
    non-existent system service object pattern. Our \codegen{} creates a template that returns an
    error by default, but AOSP and vendors can customize it to handle it more gracefully.
    % \sk{Provide some examples of what they can do.}
    For example, Jelly Bean OS added a new method named \texttt{getAnimationScale()} for a system
    service called the \textit{Window Manager}. Since Ice Cream Sandwich OS's Window Manager does not
    have the method, we wrote a translation to return the animation scale value which is
    available from the global settings.
    % \sk{Also give some experience description here, how many lines, was it difficult, etc.}
    To do so, we had to manually write only 3 lines of code.
    
%\end{enumerate}

% \dkc{we translated X out of Y mismatching SSI methods between 4.1 geust OS and 4.0 host OS, and AX out of AY methods between 8.1 guest OS and 9.0 host OS. To do so, XX object proxies, YY call translators, and ZZ pretenders. In total, they took X lines of codes but only Y lines were manually written thanks to automation. that was sufficient for testing out XXX synthetic apps and 5 poular real apps (see eval section)}

\dk{In our experience of translating SSI between JB compatibility OS and ICS host OS, we found 11 different inconsistent parcel definition patterns, 16 different inconsistent call signature patterns, one non-existent system service object pattern, and one non-existent SSI call pattern. We developed our translation code generation tool for automating each pattern with this experience. With the tool, we translated SSI between Oreo compatibility OS and Pie host OS for executing six popular commercial apps downloaded more than a billion times in the compatibility mode. To do so, we translated 61 SSI calls and 49 Parcels, and the tool generated 14,895 out of 15,259 lines of code for translation. We detail this in \cref{sec:commodity_app}.}

\subsection{SSI Translation at Run Time}
\label{sec:ssi_translation_api}

Once SSI translation code is generated, we compile and package it as SSI translation packs. They are
downloaded to a user device with a compatibility OS image. Compatibility OS's app framework loads the
packs and translates SSI calls with the packs during app execution. The translation is done within
Android's Binder, which provides us an opportunity to catch all SSI calls.


\begin{comment}
% Android's app framework and system services work together via SSI. SSI exports app framework's functionality to system services (\eg{} executing app logic) and vice versa (\eg{} acquiring system resources).
% App framework and system services must have consistent SSI definitions to make SSI calls to each other.
% They usually have the same SSI definition in a regular Android OS; however, they may not in compatibility mode as \proj{} executes app framework from compatibility OS and system services from host OS together. Two different Android OS may have different SSI definition due to AOSP's OS update and vendors' OS customization.
% When compatibility OS's app framework and host OS's system services make SSI calls to each other, the SSI calls may fail if their SSI definitions mismatch.
%\dk{Executing the app framework and the system servers from heterogeneous OS makes their communication channel, SSI, possibly fail due to the communication interface mismatch.}
%To prevent SSI call failures from SSI mismatch, 
In \proj{}, a compatibility OS uses the system services of the host OS, which means that
it uses the system services from a different OS version. This naturally creates a possibility of
interface version mismatch, \ie{} the interface of the host OS's system services might be different
from what the compatibility OS expects.

In order to address this problem, \proj{} translates system service interface (SSI) calls at run time.
%, \ie{} converting SSI calls in source SSI into SSI calls in destination SSI \dk{at run-time}.
Since SSI mismatch occurs due to AOSP's OS updates and vendors' OS customization, \proj{} asks AOSP and vendors to write their own SSI translation for their SSI changes.
Since this process of writing interface translation can be tedious, \proj{} provides a translation
code generation tool that can automate many aspects of the process, which we detail in this section.
%\proj{} compiles it into SSI translation packs and applies the SSI translation packs when SSI calls are invoked in compatibility mode.

\subsection{SSI Translation in a Nutshell}
\label{sec:ssi_translation_overview}

With \proj{}'s SSI translation API, AOSP and vendors develop translation logic for each SSI calls that they changed.
% Since SSI shares functionality between app framework and system services, 
Since SSI exports app framework's functionality to system services (\eg{} executing app logic) and vice versa (\eg{} acquiring system resources),
SSI call translation goal depends on whether the SSI call's destination has the call's intended functionality or not. If the destination does have the functionality then SSI translation should rewrite the call to be the destination's SSI calls for the same functionality.
Otherwise, SSI translation should return adequate errors to the source.


Let us discuss further with an example of AOSP's \texttt{android-9.0.0\_r1} (Pie) version compatibility OS \eat{(\texttt{9.0} to be simple)} and \texttt{android-8.1.0\_r74} (Oreo) version host OS\eat{(\texttt{8.1} to be simple)}.
Pie OS\eat{\texttt{9.0}} allows an Android device to have multiple Ethernet ports while Oreo OS\eat{\texttt{8.1}} allows at most one Ethernet port.
Therefore, ethernet manager system service in Pie\eat{\texttt{9.0}}'s SSI calls require interface name parameter for specifying an Ethernet port (\eg{} \texttt{boolean isAvailable(String interface)}) while similar calls in Oreo\eat{\texttt{8.1}} do not (\eg{} \texttt{boolean isAvailable()}). When Pie's\eat{\texttt{9.0}} app framework calls \texttt{isAvailable(String interface)} with primary Ethernet interface name, the call's translator rewrites the call to omit the name because Oreo\eat{\texttt{8.1}} has the functionality of querying the primary Ethernet port's availability, \texttt{isAvailable()}. When Pie's\eat{\texttt{9.0}} app framework calls the same SSI call with secondary or other Ethernet interface name, the call translator should return a Java exception as Pie's\eat{\texttt{9.0}} ethernet manager does for invalid interface names.

We explain the types of SSI translations and how SSI translation logic can be written in code with our SSI translation API in~\cref{sec:ssi_translation_api}.

% \subsection{SSI Translation Framework}
\subsection{SSI Translation with \proj{}}
\label{sec:ssi_translation_api}

SSI translation packs are downloaded to a user device with a compatibility OS image. Compatibility OS's app framework loads the packs and translates SSI calls with the packs during app execution. To thoroughly monitor all SSI calls without any exceptions, \proj{} uses that every SSI call is serialized into a message before leaving process boundary. All SSI call messages are sent and received via Android's Binder RPC library; therefore, \proj{} installs SSI translation hook at just before Binder RPC library sends a message and right after the library receives a message. In the hook, \proj{} executes translation logic in the translation packs for each SSI call message.

% A SSI translation pack is a library of SSI call translators, and each SSI call translator is for translating each SSI call they changed.

% \proj{} has to monitor all SSI calls 
% For translation, \proj{} uses that every SSI call is serialized into a message before leaving process boundary. SSI translation hooks are created during compatibility OS packaging. The hooks are placed at just 
% A compatibility OS's app framework loads translation packs, and it monitors \proj{} 


% \dkc{we call SSI translators at SSI translation hooks injected during compatibility OS packaging}

% \proj{} provides SSI translation API for developing a call translator for each SSI call, and it packages call translators into a translation pack. 
% \dk{A call translator essentially modifies messages for a specific SSI call;\hj{how difficult it is?} however, developers\hj{confused with app developers} can focus on high-level call semantics with our SSI translation API as the API abstracts low-level message modification details.}
% We explain what is SSI translation and how \proj{}'s SSI translation API eases it in this section.

% \proj{} translates SSI call messages; therefore, each call translator translates a SSI call message for invoking a SSI call.
\proj{} translates a SSI call by modifying SSI messages. Each SSI transaction message invokes a SSI call in a remote process.
Invoking a SSI call requires three components: a method to call, a remote object where the method belongs, and call parameters. When a SSI call is invoked, Android's RPC framework writes the three components on a transaction message. The message has three major categories of data types. One is primitive type (\eg{} integer). Another is active object, a globally unique token for a Java/C++ object implementing SSI calls. The other is Parcel, a list of primitive types, active objects, or Parcels. A Parcel represents a Java/C++ object implementing \texttt{writeToParcel()} and \texttt{createFromParcel()} methods. In the transaction message, the method becomes an integer which we call ``call ID'', the remote object becomes an active object, and the call parameters become a Parcel. A SSI call invocation is always synchronized; that means, the RPC framework always wait for a reply message after sending a transaction message. A reply message has either return values or error details (\eg{} Java exceptions) if error has occurred while handling the call.

Our SSI translation API provides \texttt{CallTranslator} class in C++ and Java for translating a SSI call. We also provide \texttt{Transaction} class and \texttt{Reply} class representing a transaction message and a reply message, respectively. \texttt{Transaction} class has a call ID field and a parameter field, and \texttt{Reply} class has a return value field. AOSP and vendors' task is implementing \texttt{CallTranslator} class for each SSI calls that they changed. They should override \texttt{CallTranslator}'s \texttt{translateTransaction(Transaction)} method for translating a transaction message by modifying \texttt{Transaction} object and override \texttt{translateReply(Reply)} method for translating a reply message by modifying \texttt{Reply} object.

% We have derived five basic SSI mismatch patterns to be handled by \texttt{CallTranslator}s. There are four variable elements in a SSI definition: interface classes holding SSI calls, SSI calls with unique names, parameters and return value signature of a SSI call, and Parcel as variable data type for parameters and return values. 

AOSP and vendors can translate a call by writing small amount of code about high-level call semantics while our \codegen{} automates low-level message modifications.
% We have developed translation patterns for each SSI mismatch pattern.
Specifically, we have identified five basic SSI mismatch patterns and developed translation patterns for each of them.
If AOSP and vendors provide two copy of Android OS source code before and after their modifications then our \codegen{} fully or partially automates writing codes in those patterns by comparing the two source codes.

\begin{figure}[!t]
    \centering
    % \begin{subfigure}[b]{\columnwidth{}}
    %     \centering
        % \scalebox{0.90}{
        \lstset{basicstyle={\scriptsize\ttfamily},
                keywordstyle=\bfseries\color{blue},
                stringstyle=\bfseries\color{olive},
                commentstyle=\bfseries\color{gray},
                morecomment=[s][\color{gray}]{@}{\ },
                numbers=left,
                aboveskip=0pt,
                belowskip=0pt}
%         \lstinputlisting[language=Java,lastline=1]{code/call_translator.txt}
%         \lstinputlisting[language=Java,firstnumber=2,firstline=2,lastline=2,backgroundcolor=\color{orange!10}]{code/call_translator.txt}
%         \lstinputlisting[language=Java,firstnumber=3,firstline=3,lastline=3]{code/call_translator.txt}
%         \lstinputlisting[language=Java,firstnumber=4,firstline=4,lastline=9,backgroundcolor=\color{orange!10}]{code/call_translator.txt}
%         \lstinputlisting[language=Java,firstnumber=10,firstline=10,lastline=26]{code/call_translator.txt}
%         \lstinputlisting[language=Java,firstnumber=27,firstline=27,lastline=29,backgroundcolor=\color{orange!10}]{code/call_translator.txt}
%         \lstinputlisting[language=Java,firstnumber=30,firstline=30]{code/call_translator.txt}
%         % } %scalebox

        % \lstinputlisting[language=Java,lastline=2]{code/call_translator_v2.txt}
        % \lstinputlisting[language=Java,firstnumber=3,firstline=3,lastline=3,backgroundcolor=\color{orange!10}]{code/call_translator_v2.txt}
        % \lstinputlisting[language=Java,firstnumber=4,firstline=4,lastline=4]{code/call_translator_v2.txt}
        % \lstinputlisting[language=Java,firstnumber=5,firstline=5,lastline=11,backgroundcolor=\color{orange!10}]{code/call_translator_v2.txt}
        % \lstinputlisting[language=Java,firstnumber=12,firstline=12,lastline=13]{code/call_translator_v2.txt}
        % \lstinputlisting[language=Java,firstnumber=14,firstline=14,lastline=16,backgroundcolor=\color{orange!10}]{code/call_translator_v2.txt}
        % \lstinputlisting[language=Java,firstnumber=17,firstline=17]{code/call_translator_v2.txt}
        
        \lstinputlisting[language=Java,lastline=2]{code/call_translator_v3.txt}
        \lstinputlisting[language=Java,firstnumber=3,firstline=3,lastline=3,backgroundcolor=\color{orange!10}]{code/call_translator_v3.txt}
        \lstinputlisting[language=Java,firstnumber=4,firstline=4,lastline=4]{code/call_translator_v3.txt}
        \lstinputlisting[language=Java,firstnumber=5,firstline=5,lastline=11,backgroundcolor=\color{orange!10}]{code/call_translator_v3.txt}
        \lstinputlisting[language=Java,firstnumber=12,firstline=12,lastline=13]{code/call_translator_v3.txt}
        \lstinputlisting[language=Java,firstnumber=14,firstline=14,lastline=16,backgroundcolor=\color{orange!10}]{code/call_translator_v3.txt}
        \lstinputlisting[language=Java,firstnumber=17,firstline=17]{code/call_translator_v3.txt}

        % } %scalebox
        % \caption{ for opening default DB file using KeePassDroid.}
        \label{fig:api_snippet}
    % \end{subfigure}
    % \hfill
%     \caption{A SSI call translator code for translating Android 9.0 OS's \texttt{isAvailable(String ifname)} to Android 8.1 OS's \texttt{isAvailable()}. Only the highlighted lines are manually written, otherwise automatically generated, and more generated code is omitted.}

    \caption{A Java SSI call translator code for translating Android 9.0's \texttt{isAvailable(String ifname)} to Android 8.1's \texttt{isAvailable()}. Only the highlighted lines are manually written, otherwise automatically generated, and more generated code is omitted.}
    \label{fig:api_example}
    
\end{figure}

\dkc{We list issue types that SSI translation have to handle. But, instead of listing them, listing how we automate/ease handling the issues may give a more positive impression to the readers.}

\begin{enumerate}[leftmargin=2\parindent]
    \item \textbf{Inconsistent call ID:}
    % \dkc{we do this automatically}
    The call ID of each SSI call is usually hard-coded in the source code, and the same SSI call in two different Android OS may have different call IDs due to the source code updates. Our \codegen{} lists all SSI calls and their IDs in each Android OS source code, and generates a \texttt{CallTranslator} modifying call ID from one SSI to call ID from another SSI if they have the same SSI call name. Hence, handling inconsistent call IDs is fully automated, and AOSP and vendors does not need to care about this type of issues.
    
    \item \textbf{Inconsistent call signature:}
    % \dkc{we generate call translator}
    A SSI call's parameters and return values might be differ by different SSIs. Since parameters are written one next to another in a message, a call translator must modify message contents to add, remove, or modify parameters. However, manually modifying message contents is error-prone and tedious in our translation experience. Our \codegen{} therefore generates a semantic call translator abstracting message modification procedure. \codegen{} reuses message serialization and deserialization code from source SSI and destination SSI. Source SSI's deserialization code converts parameter values in a message into Java variables, and destination SSI's serialization code converts translated Java variable parameters back to a message. In between deserialization and serialization, AOSP and vendors can translate call parameters and a return value in Java/C++ object form. Figure~\ref{fig:api_example} shows an example code of translating \texttt{isAvailable} SSI call example in \cref{sec:ssi_translation_overview}.
    % \cp{needs a brief explanation what the code represents, especially the bottom part which is automatically generated}

    \item \textbf{Inconsistent Parcel definition:} 
    % \dkc{we generate converter}
    A Java/C++ object parameter (or a return value) becomes a parcel when it is written to a message. It's written form might be differ by different SSIs if the SSIs define its \texttt{writeToParcel()} and \texttt{createFromParcel()} methods differently. \codegen{} automatically generates \transformer{} that transforms a Parcel in one SSI's format into another SSI's format. \transformer{} fully automates this by reading a Parcel with one SSI's \texttt{createFromParcel()} method and writing it with another SSI's \texttt{writeToParcel()} method. 

    \item \textbf{Inexistent active object:} 
    % \dkc{should create pretender}
    Every SSI call has a target remote object, and the remote object is obtained by a previous SSI call querying the remote object. However, a specific remote object type queried from one SSI may not exist in another SSI. In this case, an object faking the missing remote object can be returned instead. We call this type of object \pretender{}. AOSP and vendors should implement \pretender{} and SSI calls in it to continue translation in each SSI call; \ie{} returning error or executing proper functionality when one of the calls are invoked. \codegen{} creates \pretender{} skeleton code for AOSP and vendors.

    \item \textbf{Inexistent SSI call:} 
    % \dkc{alternative reply}
    When destination SSI does not have a SSI call invoked from source SSI, a call translator should make a reply message on behalf of destination SSI. To do so, the call translator should drop transaction message by returning \texttt{null} from \texttt{translateTransaction()} method, and compose the reply message in \texttt{translateReply()} method.
    
\end{enumerate}

In our experience of translating 47 SSI calls for Android Jelly Bean compatibility OS and Android Ice Cream Sandwich host OS, all translation cases were either one of the basic patterns or a combination of a few basic patterns.
%  \cp{In the paper, we sometimes use version numbers but sometimes mix with internal code names for Android OS version. Let's make them consistent.}
%  We describe our SSI translation experience further in \cref{sec:implementation}. \dkc{TODO: we include this???}

% \hj{

% When a transaction for an SSI call is called in the proxy, our API checks whether the same call exists in the stub.
% \begin{enumerate}
%     \item If the call does not exist in the stub (or no stub), the transaction is not passed to the stub. Developers should implement a logic to generate a reply within the proxy.
% \end{enumerate}
% If the call exists in the stub, 1) transaction parameters are passed to the stub, 2) stub executes the call with the parameters then returns a reply, and 3) the reply is passed back to the proxy. The translation is implemented to interrupt and change the transaction parameters and the reply before they are passed to the remote. The basic types for the translation are as below.
% \begin{enumerate}
%     \setcounter{enumi}{1}
%     \item If a parameter/reply disappears in the remote call, developers should drop the parameter/reply in the translation.
%     \item If a parameter/reply is newly added in the remote call, developers should generate the variable and assign a new value for it.
%     \item Even if there is no newly added or disappeared parameter/reply in the remote, the actual value in a parameter/reply may be changed. In this case, developers should assign a new value to the variable for the translation.
% \end{enumerate}
% When developers assign a new value for a parameter/reply, basically the value should be able to be derived from the 1) source parameters/reply values and 2) the stateful variables in the proxy. Developers can use a key-value store which can be used between the translator and proxy OS for easily accessing the stateful variables in the proxy.

% If we think about the primitive types like integer, float, string, or array of them, the translated values can be directly generated and assigned to the variables in the parameters/reply. However, there are two parameter types which require additional translation: parcelable objects and binders indicating interfaces. Developers should be aware of the two types, and follow the translation instructions given as below.
% \begin{enumerate}
%     \setcounter{enumi}{4}
%     \item If there is a parcelable with changed structure in the remote parameters/reply, developers should implement an independent translator for generating the remote’s parcelable object. It is for translating the intra-parcelable construction logic from the source’s to remote’s.
%     \item If the remote parameters/reply include a binder(native pointer) indicating a changed interface, developers should implement a logic to maintain a single instance of translated interface that follows the remote’s implementation. The pointer indicating the generated instance should be given as the translated parameter/reply.
% \end{enumerate}

% } % hj

\end{comment}

==> src/07_dev_study.tex <==
\section{Developer Study}
